EnduRL: Enhancing Safety, Stability, and Efficiency of Mixed Traffic Under Real-World Perturbations Via Reinforcement Learning

Human-driven vehicles (HVs) amplify naturally occurring perturbations in traffic, leading to congestion--a major contributor to increased fuel consumption, higher collision risks, and reduced road capacity utilization. While previous research demonstrates that Robot Vehicles (RVs) can be leveraged to mitigate these issues, most such studies rely on simulations with simplistic models of human car-following behaviors. In this work, we analyze real-world driving trajectories and extract a wide range of acceleration profiles. We then incorporates these profiles into simulations for training RVs to mitigate congestion. We evaluate the safety, efficiency, and stability of mixed traffic via comprehensive experiments conducted in two mixed traffic environments (Ring and Bottleneck) at various traffic densities, configurations, and RV penetration rates. The results show that under real-world perturbations, prior RV controllers experience performance degradation on all three objectives (sometimes even lower than 100% HVs). To address this, we introduce a reinforcement learning based RV that employs a congestion stage classifier to optimize the safety, efficiency, and stability of mixed traffic. Our RVs demonstrate significant improvements: safety by up to 66%, efficiency by up to 54%, and stability by up to 97%.

==> sections/prelim.tex <==
\section{Preliminaries} 
\label{sec:prelim}
% In this section, we introduce the Intelligent driver model as well as various approaches used by Robot Vehicles (RV) for traffic flow control.
% Various robot vehicles (RV), described in section~\ref{subsec:controllers} with stabilization characteristics are presented in Table~\ref{table:controllers}, have been developed to prevent the formation of stop-and-go traffic. 
% We briefly introduce IDM, \h{various RVs considered in this study, and the problem formulation for RL}. 

% \subsection{Reinforcement Learning (RL)}
% RL is a $T$-step episodic task where an agent interacts with its environment and seeks to maximize the sum of discounted rewards. At each time step, the agent is given a state $s$, responds with an action $a$, and then the environment returns the next state $s'$ and reward $r$. This is formalized as a partially observable markov decision process represented as \((\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \Omega, \mathcal{O}, \gamma)\), where \(\mathcal{S}\) represents the set of states, \(\mathcal{A}\) is the set of actions, \(\mathcal{P}(s', r | s, a)\) describes the environment dynamics, \(\mathcal{R}(s,a)\) is the reward function, \(\Omega\) represents the set of observations, \(\mathcal{O}(o | s', a)\) is the observation function defining the probability of observing \(o\) given the action \(a\) has led to state \(s'\), and \(\gamma\) is the discount factor. RL-based methods have gained popularity as an effective alternative to model-based or heuristic-based methods. 

